Neighborhood Variants of the KKM Lemma, Lebesgue Covering Theorem, and Sperner's Lemma on the Cube

We establish a "neighborhood" variant of the cubical KKM lemma and the Lebesgue covering theorem and deduce a discretized version which is a "neighborhood" variant of Sperner's lemma on the cube. The main result is the following: for any coloring of the unit $d$-cube $[0,1]^d$ in which points on opposite faces must be given different colors, and for any $\varepsilon>0$, there is an $\ell_\infty$ $\varepsilon$-ball which contains points of at least $(1+\frac{\varepsilon}{1+\varepsilon})^d$ different colors, (so in particular, at least $(1+\frac{2}{3}\varepsilon)^d$ different colors for all sensible $\varepsilon\in(0,\frac12]$).

==> _prelude/_authors.tex <==

\usepackage{authblk}

% https://tex.stackexchange.com/questions/428590/adding-email-under-author-affiliation
\makeatletter
\newcommand\email[2][]%
  {\newaffiltrue\let\AB@blk@and\AB@pand
      \if\relax#1\relax\def\AB@note{\AB@thenote}\else\def\AB@note{\relax}%
        \setcounter{Maxaffil}{0}\fi
      \begingroup
        \let\protect\@unexpandable@protect
        \def\thanks{\protect\thanks}\def\footnote{\protect\footnote}%
        \@temptokena=\expandafter{\AB@authors}%
        {\def\\{\protect\\\protect\Affilfont}\xdef\AB@temp{\url{#2}}}%
         \xdef\AB@authors{\the\@temptokena\AB@las\AB@au@str
         \protect\\[\affilsep]\protect\Affilfont\AB@temp}%
         \gdef\AB@las{}\gdef\AB@au@str{}%
        {\def\\{, \ignorespaces}\xdef\AB@temp{\url{#2}}}%
        \@temptokena=\expandafter{\AB@affillist}%
        \xdef\AB@affillist{\the\@temptokena \AB@affilsep
          \AB@affilnote{}\protect\Affilfont\AB@temp}%
      \endgroup
      \let\AB@affilsep\AB@affilsepx
}
\makeatother

\renewcommand\Authfont{}
\renewcommand\Affilfont{\itshape\small}
\setlength{\affilsep}{2em}
\setcounter{Maxaffil}{2}

\author{Jason Vander Woude}
\affil{Department of Mathematics and School of Computing, University of Nebraska-Lincoln}
\email{jasonvw@huskers.unl.edu}

\author{Peter Dixon}
\affil{Independent Researcher}
\email{tooplark@gmail.com}

\author{A. Pavan}
\affil{Department of Computer Science, Iowa State University}
\email{pavan@cs.iastate.edu}

\author{Jamie Radcliffe}
\affil{Department of Mathematics, University of Nebraska-Lincoln}
\email{aradcliffe1@unl.edu}

\author{N. V. Vinodchandran}
\affil{School of Computing, University of Nebraska-Lincoln}
\email{vinod@cse.unl.edu}



==> _prelude/_watermark.tex <==
\usepackage{draftwatermark}
% \SetWatermarkText{DRAFT}
\SetWatermarkText{DRAFT: DO NOT\\DISTRUBUTE}
\SetWatermarkLightness{0.97}
\SetWatermarkScale{3}
% \SetWatermarkScale{3.5}
